ContTune: Continuous Tuning by Conservative Bayesian Optimization for Distributed Stream Data Processing Systems

The past decade has seen rapid growth of distributed stream data processing systems. Under these systems, a stream application is realized as a Directed Acyclic Graph (DAG) of operators, where the level of parallelism of each operator has a substantial impact on its overall performance. However, finding optimal levels of parallelism remains challenging. Most existing methods are heavily coupled with the topological graph of operators, unable to efficiently tune under-provisioned jobs. They either insufficiently use previous tuning experience by treating successively tuning independently, or explore the configuration space aggressively, violating the Service Level Agreements (SLA). To address the above problems, we propose ContTune, a continuous tuning system for stream applications. It is equipped with a novel Big-small algorithm, in which the Big phase decouples the tuning from the topological graph by decomposing the job tuning problem into sub-problems that can be solved concurrently. We propose a conservative Bayesian Optimization (CBO) technique in the Small phase to speed up the tuning process by utilizing the previous observations. It leverages the state-of-the-art (SOTA) tuning method as conservative exploration to avoid SLA violations. Experimental results show that ContTune reduces up to 60.75% number of reconfigurations under synthetic workloads and up to 57.5% number of reconfigurations under real workloads, compared to the SOTA method DS2.

==> bo.tex <==
The Bayesian Optimization method introduces exploration, and the parallelism of the acquisition function selection is usually larger in confidence if it is far from the nearest sample point and is considered an aggressive exploration. 
The online tuning scenario wants to avoid aggressive exploration, and ContTune introduces the general methods that are efficient for one-shot tuning as conservative exploration. 
ContTune designs a new acquisition function to determine whether to use the parallelism chosen by the Bayesian Optimization method or general methods based on the distance of the parallelism chosen by the Bayesian Optimization method to the nearest sample point and the distance to the nearest sample point is closely related to the confidence level, which compensates the limitation of using only the mean value in the Bayesian Optimization method (Section 6.1). 
The \textit{Bayesian Optimization method}, \textit{general methods}, and the \textit{acquisition function} make up conservative Bayesian Optimization.



These works ~\cite{gulisano2012streamcloud,lohrmann2015elastic,fu2017drs,zaharia2013discretized,fischer2015machines,googleCloudDataflow2016,kalavri2018three,mei2020turbine,liu2022dragster} can be regarded as a tune using  \textit{multi-operator} pattern, and \textit{single-operator} pattern works ~\cite{castro2013integrating,heinze2014latency,xu2016stela,floratou2017dhalion,pravega2017,gedik2013elastic}. 
By the way, ContTune can use the $St_{samples}$ of other unchanged operators after some operators are changed because the tune using \textit{multi-operator} pattern is only related to tuned operator itself. 
As shown in Figure ~\ref{f1}, ContTune concurrently tunes all operators at one tuning. 

\iffalse
Inspired by the fact that the one-dimensional Subspaces Bayesian Optimization method will have better optimization results ~\cite{kirschner2019adaptive} and that horizontal tuning (tuning the parallelism of operator) has a greater improvement on the processing ability of the operator than vertical tuning (not tuning parallelism, tuning other parameters) ~\cite{roger2019comprehensive,cardellini2022runtime}, ContTune uses only parallelism as the One-Dimensional Subspaces for the Bayesian Optimization.
\fi

ContTune uses the performance model generated by GP and $St_{samples}$ that better solves the nonlinearity problem ~\cite{kalavri2018three,mei2020turbine,liu2022dragster} encountered in the current state-of-the-art methods ~\cite{kalavri2018three,mei2020turbine} of one-shot tuning.


\begin{equation}
\label{UCB}
x_t=arg\max _{x\in D}\left( \mu _{t-1}\left( x \right) +\beta ^{1/2}\sigma _{t-1}\left( x \right) \right) 
\end{equation}
LCB ~\cite{liu2014gaspad}, 
\begin{equation}
\label{LCB}
x_t=arg\max _{x\in D}\left( \mu _{t-1}\left( x \right) -\beta ^{1/2}\sigma _{t-1}\left( x \right) \right) 
\end{equation}
and EIC ~\cite{gelbart2014bayesian}, 
\begin{equation}
\begin{gathered}
\label{EIC}
y\left( x \right) \sim GP\left( \mu \left( x \right) ,k\left( x,x \right) \right) \\
PR\left( x,W \right) =P\left( y\left( x \right) \ge W \right) \\
x_t=arg\max _{x\in D}\left( \left( x^*-x \right) \times PR\left( x,W \right) \right) 
\end{gathered}
\end{equation}
and $x^*$ means the minimum parallelism that its corresponding processing ability is lager than current workload $W$ in $St_{samples}$. 
for the selection of the acquisition function in Bayesian Optimization. They all have certain problems.
For UCB, the processing ability of the operator is represented by the mean value plus the confidence level, which encourages the use of parallelism smaller than the target parallelism and tends to make job backpressure. 
For LCB, the processing ability of the operator is represented by the mean value minus the confidence level, which encourages the use of parallelism larger than the target parallelism and can result in a waste of CPU resources. 
EIC shows a certain chance of encouraging the exploration of parallelism less than the target parallelism, and once these parallelisms are attempted, additional reconfigurations are required to keep the job from backpressure. 

Formally, our acquistion function is:
\begin{equation}
\begin{gathered}
\label{OUR}
I\left( x \right) =\begin{cases}
	1&		if\ x\ge 0\\
	0&		if\ x<0\\
\end{cases} \\
x_t=arg\max _{x\in D}\left( x^*-x \right) I\left( \mu \left( x \right) -W \right) 
\end{gathered}
\end{equation}
and $x^*$ means the minimum parallelism that its corresponding processing ability is larger than current workload $W$ in $St_{samples}$. 
ContTune uses Bayesian Optimization as exploitation. 
